Future Gravitational Wave Detectors Based on Atom Interferometry

We present the perspective of using atom interferometry for gravitational wave (GW) detection in the mHz to about 10 Hz frequency band. We focus on light-pulse atom interferometers which have been subject to intense developments in the last 25 years. We calculate the effect of the GW on the atom interferometer and present in details the atomic gradiometer configuration which has retained more attention recently. The principle of such a detector is to use free falling atoms to measure the phase of a laser, which is modified by the GW. We highlight the potential benefits of using atom interferometry compared to optical interferometry as well as the challenges which remain for the realization of an atom interferometry based GW detector. We present some of the important noise sources which are expected in such detectors and strategies to cirucumvent them. Experimental techniques related to cold atom interferometers are briefly explained. We finally present the current progress and projects in this rapidly evolving field.

==> Geiger/bibliography.tex <==
\begin{thebibliography}{99}

\bibitem[{\AmS(2004)}]{ams04}
\AmS (2004). \emph{\AmS-\LaTeX{} Version 2 User's Guide} (American Mathematical
  Society, Providence), \url{http://www.ams.org/tex/amslatex.html}.

\bibitem[{Baker and Carter(1972)}]{bake72}
Baker, D.~W. and Carter, N.~L. (1972). \emph{Seismic Velocity Anisotropy
  Calculated for Ultramafic Minerals and Aggregates}, \emph{Geophys.
  Mono.}, Vol.~16 (Am. Geophys. Union), pp. 157--166.

\bibitem[{Benhamou and Colmerauer(1993)}]{benh93}
Benhamou, F. and Colmerauer, A. (eds.) (1993). \emph{Constraint Logic
  Programming, Selected Research} (MIT Press).

\bibitem[{Bestbury(2003)}]{best03}
Bestbury, B.~W. (2003). {$R$}-matrices and the magic square, \emph{J.
  Phys. A} \textbf{36}, 7, pp. 1947--1959.

\bibitem[{Brown(1988)}]{brow88}
Brown, M.~E. (1988). \emph{An interactive environment for literate
  programming}, Ph.D. thesis, Texas A\&M University, TX, USA.

\bibitem[{Churchill and Brown(1990)}]{chur90}
Churchill, R.~V. and Brown, J.~W. (1990). \emph{Complex {V}ariables and
  {A}pplications}, 5th edn. (McGraw-Hill).

\bibitem[{Davidsen(1993)}]{davi93}
Davidsen, B. (1993). Netpbm,
  \url{ftp://ftp.wustl.edu/graphics/graphics/packages/NetPBM}.

\bibitem[{Deligne and Gross(2002)}]{pier02}
Deligne, P.~X. and Gross, B.~H. (2002). On the exceptional series, and
  its descendants, \emph{C. R. Math. Acad. Sci. Paris} \textbf{335}, 11, pp.
  877--881.

\bibitem[{Gupta and Senturia(1997)}]{gupt97}
Gupta, R.~K. and Senturia, S.~D. (1997). Pull-in time dynamics as a
  measure of absolute pressure, in \emph{Proc. IEEE Int. Workshop
  on Microelectromechanical Systems (MEMS'97)} (Nagoya, Japan), pp. 290--294.

\bibitem[{Heard \emph{et~al.}(1994)Heard, Borg, Carter and Raleigh}]{hear94}
Heard, H.~C., Borg, I.~V., Carter, N.~L. and Raleigh, C.~B. (1994).
  {VoQS: Voice Quality Symbols}, Revised to 1994.

\bibitem[{Hobby(1992)}]{hobb92}
Hobby, J.~D. (1992). {A User's Manual for MetaPost}, Tech. Rep. 162,
  AT\&T Bell Laboratories, Murray Hill, New Jersey.

\bibitem[{Jarlskog(1988)}]{jarl88}
Jarlskog, C. (1988). \emph{CP {V}iolation} (World Scientific, Singapore).

\bibitem[{Jones(1973)}]{dani73}
Jones, D. (1973). {The term `phoneme'}, in W.~E. Jones and J.~Laver
  (eds.), \emph{Phonetics in Linguistics: A Book of Reading} (Longman, London),
  pp. 187--204.

\bibitem[{Kernighan(1984)}]{bria84}
Kernighan, B.~W. (1984). {PIC}---{A} graphics language for
  typesetting, Computing Science Technical Report 116, AT\&T Bell
  Laboratories, Murray Hill, New Jersey.

\bibitem[{Lamport(1987)}]{lamp87}
Lamport, L. (1987). \emph{Make Index: An Index Processor For LaTeX}.

\bibitem[{Lamport(1994)}]{lamp94}
Lamport, L. (1994). \emph{\LaTeX, A Document Preparation System}, 2nd edn.
  (Addison-Wesley, Reading, MA).

\bibitem[{Landsberg and Manivel(2002)}]{jame02}
Landsberg, J.~M. and Manivel, L. (2002). Triality, exceptional {L}ie
  algebras and {D}eligne dimension formulas, \emph{Adv. Math.} \textbf{171},
  1, pp. 59--85, \url{http://www.url.com/triality.html}.

\bibitem[{Lodha(1974)}]{lodh74}
Lodha, G.~S. (1974). \emph{Quantitative interpretation of ariborne
  electromagnetic response for a spherical model}, Master's thesis, University
  of Toronto, Canada.

\bibitem[{Richardson(1960)}]{rich60}
Richardson, L.~F. (1960). \emph{Arms and {I}nsecurity} (Boxwood, Pittsburg).

\bibitem[{Weiss(1994)}]{weis94}
Weiss, G.~H. (ed.) (1994). \emph{Contemporary {P}roblems in {S}tatistical
  {P}hysics} (SIAM, Philadelphia).

\end{thebibliography}

